On the Erdos Discrepancy Problem

According to the Erd\H{o}s discrepancy conjecture, for any infinite $\pm 1$ sequence, there exists a homogeneous arithmetic progression of unbounded discrepancy. In other words, for any $\pm 1$ sequence $(x_1,x_2,...)$ and a discrepancy $C$, there exist integers $m$ and $d$ such that $|\sum_{i=1}^m x_{i \cdot d}| > C$. This is an $80$-year-old open problem and recent development proved that this conjecture is true for discrepancies up to $2$. Paul Erd\H{o}s also conjectured that this property of unbounded discrepancy even holds for the restricted case of completely multiplicative sequences (CMSs), namely sequences $(x_1,x_2,...)$ where $x_{a \cdot b} = x_{a} \cdot x_{b}$ for any $a,b \geq 1$. The longest CMS with discrepancy $2$ has been proven to be of size $246$. In this paper, we prove that any completely multiplicative sequence of size $127,646$ or more has discrepancy at least $4$, proving the Erd\H{o}s discrepancy conjecture for CMSs of discrepancies up to $3$. In addition, we prove that this bound is tight and increases the size of the longest known sequence of discrepancy $3$ from $17,000$ to $127,645$. Finally, we provide inductive construction rules as well as streamlining methods to improve the lower bounds for sequences of higher discrepancies.

==> Makefile <==
.PHONY: main tar fromscratch dvi ps pdf bibs figs compact clean

TEXFILE    = materialsdiscoverydataset

LATEX      = latex
BIBTEX     = bibtex
MAKEINDEX  = makeindex
DVIPS      = dvips -t letter
PDFLATEX   = pdflatex
FIGDIR     = figs
CURRENTDIR = `basename "\`pwd\`"`

main: pdf

tar:
	rm -f ../$(CURRENTDIR).tar.gz
	tar cvf ../$(CURRENTDIR).tar ../$(CURRENTDIR)
	gzip ../$(CURRENTDIR).tar
	echo "Created ../$(CURRENTDIR).tar.gz"

tgz:
	rm -f ../$(CURRENTDIR).tgz
	tar cvfz ../$(CURRENTDIR).tgz ../$(CURRENTDIR)
	echo "Created ../$(CURRENTDIR).tgz"

#fromscratch: figs
fromscratch:
	$(LATEX) $(TEXFILE)
	$(BIBTEX) $(TEXFILE)
	$(LATEX) $(TEXFILE)
	$(LATEX) $(TEXFILE)
	$(DVIPS) $(TEXFILE).dvi -o $(TEXFILE).ps

dvi:
	$(LATEX) $(TEXFILE)

ps: dvi
	$(DVIPS) $(TEXFILE).dvi -o $(TEXFILE).ps

pdf:
	$(PDFLATEX) $(TEXFILE)

bibs:
	$(BIBTEX) $(TEXFILE)

index:
	$(MAKEINDEX) $(TEXFILE)

figs:
	(cd $(FIGDIR); bash ./makefigs ../*.tex )

compact:
#	(rm -f *.aux *.log *.blg *.out *.toc $(TEXFILE).bbl)
	(rm -f *.aux *.log *.blg *.out *.toc)

clean: compact
#	(rm -f *.dvi *.ps *.pdf $(FIGDIR)/*.{eps,pdf,pstex,pstex_t,fig.bak} )
	(rm -f *.dvi *.ps *.pdf $(TEXFILE).bbl $(FIGDIR)/*.{eps,pdf,pstex,pstex_t,fig.bak} )


